Hierarchical Preemptive Holistic Collaborative Systems for Embodied Multi-Agent Systems: Framework, Hybrid Stability, and Scalability Analysis

The coordination of Embodied Multi-Agent Systems in constrained physical environments requires a rigorous balance between safety, scalability, and efficiency. Traditional decentralized approaches, e.g., reactive collision avoidance, are prone to local minima or reciprocal yielding standoffs due to the lack of future intent awareness. In contrast, centralized planning suffers from intractable computational complexity and single-point-of-failure vulnerabilities. To address these limitations, we propose the Hierarchical Preemptive Holistic Collaborative (Prollect) framework, which generalizes the Preemptive Holistic Collaborative System (PHCS) by decomposing the global coordination problem into topologically connected subspace optimizations. We formalize the system as a Hybrid Automaton and introduce a three-stage receding horizon mechanism (frozen execution, preliminary planning, proactive look-ahead windows) with explicit padding to prevent races between coordination dissemination and intent updates. Notably, we design a robust timing protocol with a mandatory Idle Buffer that acts as a dwell-time constraint to eliminate Zeno behaviors and ensure computational stability under jitter. Furthermore, we formalize a Shadow Agent protocol to guarantee seamless trajectory consistency across subspace boundaries, which we treat as an Input-to-State Stability (ISS) problem.

==> sim/results/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.19, lower quartile=1.19, median=1.19, upper quartile=1.19, upper whisker=1.19}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.30, lower quartile=1.30, median=1.30, upper quartile=1.30, upper whisker=1.30}}] coordinates {};
% intersection / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=70.90, lower quartile=70.90, median=70.90, upper quartile=70.90, upper whisker=70.90}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.25, lower quartile=1.25, median=1.25, upper quartile=1.25, upper whisker=1.25}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=53.67, median=53.97, upper quartile=54.41, upper whisker=56.95}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.20, lower quartile=1.22, median=1.24, upper quartile=1.25, upper whisker=1.27}}] coordinates {};
% bottleneck / orca - completion_time
\addplot[boxplot prepared={{lower whisker=72.65, lower quartile=72.65, median=72.65, upper quartile=72.65, upper whisker=72.65}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.26, lower quartile=1.27, median=1.28, upper quartile=1.30, upper whisker=1.32}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=52.95, lower quartile=53.36, median=53.82, upper quartile=54.52, upper whisker=56.20}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.24, lower quartile=1.26, median=1.27, upper quartile=1.27, upper whisker=1.30}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.07, median=54.35, upper quartile=54.60, upper whisker=56.65}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.19, lower quartile=1.23, median=1.24, upper quartile=1.25, upper whisker=1.26}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.90, median=52.75, upper quartile=56.95, upper whisker=63.55}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.17, lower quartile=1.24, median=1.24, upper quartile=1.25, upper whisker=1.27}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=51.32, median=54.20, upper quartile=59.02, upper whisker=74.75}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.29, median=1.30, upper quartile=1.32, upper whisker=1.61}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.99, median=52.77, upper quartile=55.57, upper whisker=63.55}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.24, lower quartile=1.27, median=1.28, upper quartile=1.28, upper whisker=1.29}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.50, median=52.75, upper quartile=56.95, upper whisker=63.55}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.20, lower quartile=1.24, median=1.24, upper quartile=1.26, upper whisker=1.28}}] coordinates {};


==> sim/results/latex_comm_sweep_table.tex <==
% Auto-generated comm sweep table (\input{sim/results/latex_comm_sweep_table.tex})
\begin{table}[t]
\caption{Communication robustness sweep (intersection, 30 seeds): completion and collision rates (\%) under i.i.d. Bernoulli packet drops with probability $p_{drop}$ and fixed delivery delay of one control cycle ($t_{tx}=t_{step}$).}
\centering\scriptsize
\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lccc@{}}\toprule
$p_{drop}$ & $\alpha=1$ (Comp/Coll) & $\alpha=3$ (Comp/Coll) & $\alpha=5$ (Comp/Coll) \\ \midrule
0.0 & 100.0/0.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.1 & 96.7/3.3 & 100.0/0.0 & 100.0/0.0 \\ 
0.2 & 23.3/6.7 & 100.0/0.0 & 100.0/0.0 \\ 
0.3 & 0.0/10.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.4 & 0.0/20.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.5 & 0.0/10.0 & 96.7/0.0 & 100.0/0.0 \\ 
\bottomrule\end{tabular}
\label{tab:comm_sweep}
\end{table}


==> sim/results_comm_smoke/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - completion_time
\addplot[boxplot prepared={{lower whisker=81.90, lower quartile=81.90, median=81.90, upper quartile=81.90, upper whisker=81.90}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.15, lower quartile=1.15, median=1.15, upper quartile=1.15, upper whisker=1.15}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.00, median=54.15, upper quartile=55.02, upper whisker=57.50}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.42, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.11, lower quartile=1.13, median=1.15, upper quartile=1.15, upper whisker=1.32}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=56.75, lower quartile=57.94, median=58.50, upper quartile=59.44, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.28, upper quartile=1.29, upper whisker=1.47}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.07, median=54.35, upper quartile=54.60, upper whisker=56.65}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.19, lower quartile=1.23, median=1.24, upper quartile=1.25, upper whisker=1.26}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.65, median=52.50, upper quartile=57.30, upper whisker=63.55}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.41, lower quartile=1.43, median=1.44, upper quartile=1.45, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=51.40, median=54.25, upper quartile=59.90, upper whisker=74.75}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.13, lower quartile=1.15, median=1.17, upper quartile=1.31, upper whisker=1.61}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=42.80, lower quartile=51.89, median=53.65, upper quartile=56.24, upper whisker=64.95}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.28, lower quartile=1.30, median=1.33, upper quartile=1.64, upper whisker=2.22}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.50, median=52.75, upper quartile=56.95, upper whisker=63.55}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.20, lower quartile=1.24, median=1.24, upper quartile=1.26, upper whisker=1.28}}] coordinates {};


==> sim/results_comm_smoke/latex_comm_sweep_table.tex <==
% Auto-generated comm sweep table (\input{sim/results/latex_comm_sweep_table.tex})
\begin{table}[t]
\caption{Communication robustness sweep (intersection, 5 seeds): completion and collision rates (\%) under i.i.d. Bernoulli packet drops with probability $p_{drop}$ and fixed delivery delay of one control cycle ($t_{tx}=t_{step}$).}
\centering\scriptsize
\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lccc@{}}\toprule
$p_{drop}$ & $\alpha=1$ (Comp/Coll) & $\alpha=3$ (Comp/Coll) & $\alpha=5$ (Comp/Coll) \\ \midrule
0.0 & 100.0/0.0 & 100.0/100.0 & 100.0/100.0 \\ 
0.1 & 100.0/0.0 & 100.0/80.0 & 100.0/100.0 \\ 
0.2 & 100.0/0.0 & 100.0/40.0 & 100.0/100.0 \\ 
0.3 & 0.0/0.0 & 100.0/40.0 & 100.0/100.0 \\ 
0.4 & 0.0/0.0 & 100.0/80.0 & 100.0/100.0 \\ 
0.5 & 0.0/0.0 & 100.0/60.0 & 100.0/100.0 \\ 
\bottomrule\end{tabular}
\label{tab:comm_sweep}
\end{table}


==> sim/results_comm_smoke/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 100.0\% & 0.0\% & 81.90 [81.90, 81.90] & 1.15 [1.15, 1.15] & 0.134 [0.134, 0.134] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.15 [54.00, 55.02] & 1.43 [1.42, 1.44] & 0.022 [0.016, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.15 [1.13, 1.15] & 0.511 [0.461, 0.550] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.50 [57.94, 59.44] & 1.28 [1.28, 1.29] & 0.199 [0.182, 0.222] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.35 [54.07, 54.60] & 1.24 [1.23, 1.25] & 0.019 [0.013, 0.026] & 0.079 [0.047, 0.115] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 96.7\% & 0.0\% & 52.50 [50.65, 57.30] & 1.44 [1.43, 1.45] & 0.024 [0.015, 0.036] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 90.0\% & 0.0\% & 54.25 [51.40, 59.90] & 1.17 [1.15, 1.31] & 0.127 [0.089, 0.150] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 53.65 [51.89, 56.24] & 1.33 [1.30, 1.64] & 0.568 [0.512, 0.618] & 0.000 [0.000, 0.000] \\ 
Prollect & 96.7\% & 0.0\% & 52.75 [50.50, 56.95] & 1.24 [1.24, 1.26] & 0.020 [0.010, 0.030] & 0.039 [0.027, 0.049] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_comm_smoke2/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - completion_time
\addplot[boxplot prepared={{lower whisker=81.90, lower quartile=81.90, median=81.90, upper quartile=81.90, upper whisker=81.90}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.15, lower quartile=1.15, median=1.15, upper quartile=1.15, upper whisker=1.15}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.00, median=54.15, upper quartile=55.02, upper whisker=57.50}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.42, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.11, lower quartile=1.13, median=1.15, upper quartile=1.15, upper whisker=1.32}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=56.75, lower quartile=57.94, median=58.50, upper quartile=59.44, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.28, upper quartile=1.29, upper whisker=1.47}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.07, median=54.35, upper quartile=54.60, upper whisker=56.65}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.19, lower quartile=1.23, median=1.24, upper quartile=1.25, upper whisker=1.26}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.65, median=52.50, upper quartile=57.30, upper whisker=63.55}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.41, lower quartile=1.43, median=1.44, upper quartile=1.45, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=51.40, median=54.25, upper quartile=59.90, upper whisker=74.75}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.13, lower quartile=1.15, median=1.17, upper quartile=1.31, upper whisker=1.61}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=42.80, lower quartile=51.89, median=53.65, upper quartile=56.24, upper whisker=64.95}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.28, lower quartile=1.30, median=1.33, upper quartile=1.64, upper whisker=2.22}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.50, median=52.75, upper quartile=56.95, upper whisker=63.55}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.20, lower quartile=1.24, median=1.24, upper quartile=1.26, upper whisker=1.28}}] coordinates {};


==> sim/results_comm_smoke2/latex_comm_sweep_table.tex <==
% Auto-generated comm sweep table (\input{sim/results/latex_comm_sweep_table.tex})
\begin{table}[t]
\caption{Communication robustness sweep (intersection, 5 seeds): completion and collision rates (\%) under i.i.d. Bernoulli packet drops with probability $p_{drop}$ and fixed delivery delay of one control cycle ($t_{tx}=t_{step}$).}
\centering\scriptsize
\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lccc@{}}\toprule
$p_{drop}$ & $\alpha=1$ (Comp/Coll) & $\alpha=3$ (Comp/Coll) & $\alpha=5$ (Comp/Coll) \\ \midrule
0.0 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.1 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.2 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.3 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.4 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.5 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
\bottomrule\end{tabular}
\label{tab:comm_sweep}
\end{table}


==> sim/results_comm_smoke2/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 100.0\% & 0.0\% & 81.90 [81.90, 81.90] & 1.15 [1.15, 1.15] & 0.134 [0.134, 0.134] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.15 [54.00, 55.02] & 1.43 [1.42, 1.44] & 0.022 [0.016, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.15 [1.13, 1.15] & 0.511 [0.461, 0.550] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.50 [57.94, 59.44] & 1.28 [1.28, 1.29] & 0.199 [0.182, 0.222] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.35 [54.07, 54.60] & 1.24 [1.23, 1.25] & 0.019 [0.013, 0.026] & 0.079 [0.047, 0.115] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 96.7\% & 0.0\% & 52.50 [50.65, 57.30] & 1.44 [1.43, 1.45] & 0.024 [0.015, 0.036] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 90.0\% & 0.0\% & 54.25 [51.40, 59.90] & 1.17 [1.15, 1.31] & 0.127 [0.089, 0.150] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 53.65 [51.89, 56.24] & 1.33 [1.30, 1.64] & 0.568 [0.512, 0.618] & 0.000 [0.000, 0.000] \\ 
Prollect & 96.7\% & 0.0\% & 52.75 [50.50, 56.95] & 1.24 [1.24, 1.26] & 0.020 [0.010, 0.030] & 0.039 [0.027, 0.049] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_comm_smoke3/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - completion_time
\addplot[boxplot prepared={{lower whisker=81.90, lower quartile=81.90, median=81.90, upper quartile=81.90, upper whisker=81.90}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.15, lower quartile=1.15, median=1.15, upper quartile=1.15, upper whisker=1.15}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.00, median=54.15, upper quartile=55.02, upper whisker=57.50}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.42, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.11, lower quartile=1.13, median=1.15, upper quartile=1.15, upper whisker=1.32}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=56.75, lower quartile=57.94, median=58.50, upper quartile=59.44, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.28, upper quartile=1.29, upper whisker=1.47}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.07, median=54.35, upper quartile=54.60, upper whisker=56.65}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.19, lower quartile=1.23, median=1.24, upper quartile=1.25, upper whisker=1.26}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.65, median=52.50, upper quartile=57.30, upper whisker=63.55}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.41, lower quartile=1.43, median=1.44, upper quartile=1.45, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=51.40, median=54.25, upper quartile=59.90, upper whisker=74.75}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.13, lower quartile=1.15, median=1.17, upper quartile=1.31, upper whisker=1.61}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=42.80, lower quartile=51.89, median=53.65, upper quartile=56.24, upper whisker=64.95}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.28, lower quartile=1.30, median=1.33, upper quartile=1.64, upper whisker=2.22}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.50, median=52.75, upper quartile=56.95, upper whisker=63.55}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.20, lower quartile=1.24, median=1.24, upper quartile=1.26, upper whisker=1.28}}] coordinates {};


==> sim/results_comm_smoke3/latex_comm_sweep_table.tex <==
% Auto-generated comm sweep table (\input{sim/results/latex_comm_sweep_table.tex})
\begin{table}[t]
\caption{Communication robustness sweep (intersection, 5 seeds): completion and collision rates (\%) under i.i.d. Bernoulli packet drops with probability $p_{drop}$ and fixed delivery delay of one control cycle ($t_{tx}=t_{step}$).}
\centering\scriptsize
\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lccc@{}}\toprule
$p_{drop}$ & $\alpha=1$ (Comp/Coll) & $\alpha=3$ (Comp/Coll) & $\alpha=5$ (Comp/Coll) \\ \midrule
0.0 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.1 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.2 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.3 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.4 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.5 & 0.0/0.0 & 0.0/40.0 & 0.0/60.0 \\ 
\bottomrule\end{tabular}
\label{tab:comm_sweep}
\end{table}


==> sim/results_comm_smoke3/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 100.0\% & 0.0\% & 81.90 [81.90, 81.90] & 1.15 [1.15, 1.15] & 0.134 [0.134, 0.134] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.15 [54.00, 55.02] & 1.43 [1.42, 1.44] & 0.022 [0.016, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.15 [1.13, 1.15] & 0.511 [0.461, 0.550] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.50 [57.94, 59.44] & 1.28 [1.28, 1.29] & 0.199 [0.182, 0.222] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.35 [54.07, 54.60] & 1.24 [1.23, 1.25] & 0.019 [0.013, 0.026] & 0.079 [0.047, 0.115] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 96.7\% & 0.0\% & 52.50 [50.65, 57.30] & 1.44 [1.43, 1.45] & 0.024 [0.015, 0.036] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 90.0\% & 0.0\% & 54.25 [51.40, 59.90] & 1.17 [1.15, 1.31] & 0.127 [0.089, 0.150] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 53.65 [51.89, 56.24] & 1.33 [1.30, 1.64] & 0.568 [0.512, 0.618] & 0.000 [0.000, 0.000] \\ 
Prollect & 96.7\% & 0.0\% & 52.75 [50.50, 56.95] & 1.24 [1.24, 1.26] & 0.020 [0.010, 0.030] & 0.039 [0.027, 0.049] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_comm_smoke4/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - completion_time
\addplot[boxplot prepared={{lower whisker=81.90, lower quartile=81.90, median=81.90, upper quartile=81.90, upper whisker=81.90}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.15, lower quartile=1.15, median=1.15, upper quartile=1.15, upper whisker=1.15}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.00, median=54.15, upper quartile=55.02, upper whisker=57.50}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.42, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.11, lower quartile=1.13, median=1.15, upper quartile=1.15, upper whisker=1.32}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=56.75, lower quartile=57.94, median=58.50, upper quartile=59.44, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.28, upper quartile=1.29, upper whisker=1.47}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.07, median=54.35, upper quartile=54.60, upper whisker=56.65}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.19, lower quartile=1.23, median=1.24, upper quartile=1.25, upper whisker=1.26}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.65, median=52.50, upper quartile=57.30, upper whisker=63.55}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.41, lower quartile=1.43, median=1.44, upper quartile=1.45, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=51.40, median=54.25, upper quartile=59.90, upper whisker=74.75}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.13, lower quartile=1.15, median=1.17, upper quartile=1.31, upper whisker=1.61}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=42.80, lower quartile=51.89, median=53.65, upper quartile=56.24, upper whisker=64.95}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.28, lower quartile=1.30, median=1.33, upper quartile=1.64, upper whisker=2.22}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.50, median=52.75, upper quartile=56.95, upper whisker=63.55}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.20, lower quartile=1.24, median=1.24, upper quartile=1.26, upper whisker=1.28}}] coordinates {};


==> sim/results_comm_smoke4/latex_comm_sweep_table.tex <==
% Auto-generated comm sweep table (\input{sim/results/latex_comm_sweep_table.tex})
\begin{table}[t]
\caption{Communication robustness sweep (intersection, 5 seeds): completion and collision rates (\%) under i.i.d. Bernoulli packet drops with probability $p_{drop}$ and fixed delivery delay of one control cycle ($t_{tx}=t_{step}$).}
\centering\scriptsize
\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lccc@{}}\toprule
$p_{drop}$ & $\alpha=1$ (Comp/Coll) & $\alpha=3$ (Comp/Coll) & $\alpha=5$ (Comp/Coll) \\ \midrule
0.0 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.1 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.2 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.3 & 0.0/0.0 & 0.0/0.0 & 0.0/0.0 \\ 
0.4 & 0.0/0.0 & 0.0/40.0 & 0.0/20.0 \\ 
0.5 & 0.0/0.0 & 0.0/40.0 & 0.0/40.0 \\ 
\bottomrule\end{tabular}
\label{tab:comm_sweep}
\end{table}


==> sim/results_comm_smoke4/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 100.0\% & 0.0\% & 81.90 [81.90, 81.90] & 1.15 [1.15, 1.15] & 0.134 [0.134, 0.134] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.15 [54.00, 55.02] & 1.43 [1.42, 1.44] & 0.022 [0.016, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.15 [1.13, 1.15] & 0.511 [0.461, 0.550] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.50 [57.94, 59.44] & 1.28 [1.28, 1.29] & 0.199 [0.182, 0.222] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.35 [54.07, 54.60] & 1.24 [1.23, 1.25] & 0.019 [0.013, 0.026] & 0.079 [0.047, 0.115] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 96.7\% & 0.0\% & 52.50 [50.65, 57.30] & 1.44 [1.43, 1.45] & 0.024 [0.015, 0.036] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 90.0\% & 0.0\% & 54.25 [51.40, 59.90] & 1.17 [1.15, 1.31] & 0.127 [0.089, 0.150] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 53.65 [51.89, 56.24] & 1.33 [1.30, 1.64] & 0.568 [0.512, 0.618] & 0.000 [0.000, 0.000] \\ 
Prollect & 96.7\% & 0.0\% & 52.75 [50.50, 56.95] & 1.24 [1.24, 1.26] & 0.020 [0.010, 0.030] & 0.039 [0.027, 0.049] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_comm_smoke5/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - completion_time
\addplot[boxplot prepared={{lower whisker=81.90, lower quartile=81.90, median=81.90, upper quartile=81.90, upper whisker=81.90}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.15, lower quartile=1.15, median=1.15, upper quartile=1.15, upper whisker=1.15}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.00, median=54.15, upper quartile=55.02, upper whisker=57.50}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.42, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.11, lower quartile=1.13, median=1.15, upper quartile=1.15, upper whisker=1.32}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=56.75, lower quartile=57.94, median=58.50, upper quartile=59.44, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.28, upper quartile=1.29, upper whisker=1.47}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.07, median=54.35, upper quartile=54.60, upper whisker=56.65}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.19, lower quartile=1.23, median=1.24, upper quartile=1.25, upper whisker=1.26}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.65, median=52.50, upper quartile=57.30, upper whisker=63.55}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.41, lower quartile=1.43, median=1.44, upper quartile=1.45, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=51.40, median=54.25, upper quartile=59.90, upper whisker=74.75}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.13, lower quartile=1.15, median=1.17, upper quartile=1.31, upper whisker=1.61}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=42.80, lower quartile=51.89, median=53.65, upper quartile=56.24, upper whisker=64.95}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.28, lower quartile=1.30, median=1.33, upper quartile=1.64, upper whisker=2.22}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.50, median=52.75, upper quartile=56.95, upper whisker=63.55}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.20, lower quartile=1.24, median=1.24, upper quartile=1.26, upper whisker=1.28}}] coordinates {};


==> sim/results_comm_smoke5/latex_comm_sweep_table.tex <==
% Auto-generated comm sweep table (\input{sim/results/latex_comm_sweep_table.tex})
\begin{table}[t]
\caption{Communication robustness sweep (intersection, 5 seeds): completion and collision rates (\%) under i.i.d. Bernoulli packet drops with probability $p_{drop}$ and fixed delivery delay of one control cycle ($t_{tx}=t_{step}$).}
\centering\scriptsize
\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lccc@{}}\toprule
$p_{drop}$ & $\alpha=1$ (Comp/Coll) & $\alpha=3$ (Comp/Coll) & $\alpha=5$ (Comp/Coll) \\ \midrule
0.0 & 100.0/0.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.1 & 100.0/20.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.2 & 20.0/40.0 & 100.0/20.0 & 100.0/0.0 \\ 
0.3 & 0.0/20.0 & 100.0/60.0 & 100.0/0.0 \\ 
0.4 & 0.0/40.0 & 100.0/80.0 & 100.0/20.0 \\ 
0.5 & 0.0/100.0 & 100.0/80.0 & 100.0/80.0 \\ 
\bottomrule\end{tabular}
\label{tab:comm_sweep}
\end{table}


==> sim/results_comm_smoke5/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 100.0\% & 0.0\% & 81.90 [81.90, 81.90] & 1.15 [1.15, 1.15] & 0.134 [0.134, 0.134] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.15 [54.00, 55.02] & 1.43 [1.42, 1.44] & 0.022 [0.016, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.15 [1.13, 1.15] & 0.511 [0.461, 0.550] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.50 [57.94, 59.44] & 1.28 [1.28, 1.29] & 0.199 [0.182, 0.222] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.35 [54.07, 54.60] & 1.24 [1.23, 1.25] & 0.019 [0.013, 0.026] & 0.079 [0.047, 0.115] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 96.7\% & 0.0\% & 52.50 [50.65, 57.30] & 1.44 [1.43, 1.45] & 0.024 [0.015, 0.036] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 90.0\% & 0.0\% & 54.25 [51.40, 59.90] & 1.17 [1.15, 1.31] & 0.127 [0.089, 0.150] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 53.65 [51.89, 56.24] & 1.33 [1.30, 1.64] & 0.568 [0.512, 0.618] & 0.000 [0.000, 0.000] \\ 
Prollect & 96.7\% & 0.0\% & 52.75 [50.50, 56.95] & 1.24 [1.24, 1.26] & 0.020 [0.010, 0.030] & 0.039 [0.027, 0.049] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_comm_smoke6/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - completion_time
\addplot[boxplot prepared={{lower whisker=81.90, lower quartile=81.90, median=81.90, upper quartile=81.90, upper whisker=81.90}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.15, lower quartile=1.15, median=1.15, upper quartile=1.15, upper whisker=1.15}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.00, median=54.15, upper quartile=55.02, upper whisker=57.50}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.42, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.11, lower quartile=1.13, median=1.15, upper quartile=1.15, upper whisker=1.32}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=56.75, lower quartile=57.94, median=58.50, upper quartile=59.44, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.28, upper quartile=1.29, upper whisker=1.47}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.07, median=54.35, upper quartile=54.60, upper whisker=56.65}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.19, lower quartile=1.23, median=1.24, upper quartile=1.25, upper whisker=1.26}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.65, median=52.50, upper quartile=57.30, upper whisker=63.55}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.41, lower quartile=1.43, median=1.44, upper quartile=1.45, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=51.40, median=54.25, upper quartile=59.90, upper whisker=74.75}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.13, lower quartile=1.15, median=1.17, upper quartile=1.31, upper whisker=1.61}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=42.80, lower quartile=51.89, median=53.65, upper quartile=56.24, upper whisker=64.95}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.28, lower quartile=1.30, median=1.33, upper quartile=1.64, upper whisker=2.22}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.50, median=52.75, upper quartile=56.95, upper whisker=63.55}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.20, lower quartile=1.24, median=1.24, upper quartile=1.26, upper whisker=1.28}}] coordinates {};


==> sim/results_comm_smoke6/latex_comm_sweep_table.tex <==
% Auto-generated comm sweep table (\input{sim/results/latex_comm_sweep_table.tex})
\begin{table}[t]
\caption{Communication robustness sweep (intersection, 10 seeds): completion and collision rates (\%) under i.i.d. Bernoulli packet drops with probability $p_{drop}$ and fixed delivery delay of one control cycle ($t_{tx}=t_{step}$).}
\centering\scriptsize
\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lccc@{}}\toprule
$p_{drop}$ & $\alpha=1$ (Comp/Coll) & $\alpha=3$ (Comp/Coll) & $\alpha=5$ (Comp/Coll) \\ \midrule
0.0 & 100.0/0.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.1 & 100.0/10.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.2 & 10.0/10.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.3 & 0.0/10.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.4 & 0.0/30.0 & 100.0/0.0 & 100.0/10.0 \\ 
0.5 & 0.0/10.0 & 100.0/0.0 & 100.0/0.0 \\ 
\bottomrule\end{tabular}
\label{tab:comm_sweep}
\end{table}


==> sim/results_comm_smoke6/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 100.0\% & 0.0\% & 81.90 [81.90, 81.90] & 1.15 [1.15, 1.15] & 0.134 [0.134, 0.134] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.15 [54.00, 55.02] & 1.43 [1.42, 1.44] & 0.022 [0.016, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.15 [1.13, 1.15] & 0.511 [0.461, 0.550] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.50 [57.94, 59.44] & 1.28 [1.28, 1.29] & 0.199 [0.182, 0.222] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.35 [54.07, 54.60] & 1.24 [1.23, 1.25] & 0.019 [0.013, 0.026] & 0.079 [0.047, 0.115] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 96.7\% & 0.0\% & 52.50 [50.65, 57.30] & 1.44 [1.43, 1.45] & 0.024 [0.015, 0.036] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 90.0\% & 0.0\% & 54.25 [51.40, 59.90] & 1.17 [1.15, 1.31] & 0.127 [0.089, 0.150] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 53.65 [51.89, 56.24] & 1.33 [1.30, 1.64] & 0.568 [0.512, 0.618] & 0.000 [0.000, 0.000] \\ 
Prollect & 96.7\% & 0.0\% & 52.75 [50.50, 56.95] & 1.24 [1.24, 1.26] & 0.020 [0.010, 0.030] & 0.039 [0.027, 0.049] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_comm_smoke7/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - completion_time
\addplot[boxplot prepared={{lower whisker=81.90, lower quartile=81.90, median=81.90, upper quartile=81.90, upper whisker=81.90}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.15, lower quartile=1.15, median=1.15, upper quartile=1.15, upper whisker=1.15}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.00, median=54.15, upper quartile=55.02, upper whisker=57.50}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.42, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.11, lower quartile=1.13, median=1.15, upper quartile=1.15, upper whisker=1.32}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=56.75, lower quartile=57.94, median=58.50, upper quartile=59.44, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.28, upper quartile=1.29, upper whisker=1.47}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.10, lower quartile=54.07, median=54.35, upper quartile=54.60, upper whisker=56.65}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.19, lower quartile=1.23, median=1.24, upper quartile=1.25, upper whisker=1.26}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.65, median=52.50, upper quartile=57.30, upper whisker=63.55}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.41, lower quartile=1.43, median=1.44, upper quartile=1.45, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=51.40, median=54.25, upper quartile=59.90, upper whisker=74.75}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.13, lower quartile=1.15, median=1.17, upper quartile=1.31, upper whisker=1.61}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=42.80, lower quartile=51.89, median=53.65, upper quartile=56.24, upper whisker=64.95}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.28, lower quartile=1.30, median=1.33, upper quartile=1.64, upper whisker=2.22}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=41.55, lower quartile=50.50, median=52.75, upper quartile=56.95, upper whisker=63.55}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.20, lower quartile=1.24, median=1.24, upper quartile=1.26, upper whisker=1.28}}] coordinates {};


==> sim/results_comm_smoke7/latex_comm_sweep_table.tex <==
% Auto-generated comm sweep table (\input{sim/results/latex_comm_sweep_table.tex})
\begin{table}[t]
\caption{Communication robustness sweep (intersection, 10 seeds): completion and collision rates (\%) under i.i.d. Bernoulli packet drops with probability $p_{drop}$ and fixed delivery delay of one control cycle ($t_{tx}=t_{step}$).}
\centering\scriptsize
\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lccc@{}}\toprule
$p_{drop}$ & $\alpha=1$ (Comp/Coll) & $\alpha=3$ (Comp/Coll) & $\alpha=5$ (Comp/Coll) \\ \midrule
0.0 & 100.0/0.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.1 & 100.0/10.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.2 & 10.0/10.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.3 & 0.0/10.0 & 100.0/0.0 & 100.0/0.0 \\ 
0.4 & 0.0/30.0 & 100.0/0.0 & 100.0/10.0 \\ 
0.5 & 0.0/10.0 & 100.0/0.0 & 100.0/0.0 \\ 
\bottomrule\end{tabular}
\label{tab:comm_sweep}
\end{table}


==> sim/results_comm_smoke7/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 100.0\% & 0.0\% & 81.90 [81.90, 81.90] & 1.15 [1.15, 1.15] & 0.134 [0.134, 0.134] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.15 [54.00, 55.02] & 1.43 [1.42, 1.44] & 0.022 [0.016, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.15 [1.13, 1.15] & 0.511 [0.461, 0.550] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.50 [57.94, 59.44] & 1.28 [1.28, 1.29] & 0.199 [0.182, 0.222] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.35 [54.07, 54.60] & 1.24 [1.23, 1.25] & 0.019 [0.013, 0.026] & 0.079 [0.047, 0.115] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 96.7\% & 0.0\% & 52.50 [50.65, 57.30] & 1.44 [1.43, 1.45] & 0.024 [0.015, 0.036] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 90.0\% & 0.0\% & 54.25 [51.40, 59.90] & 1.17 [1.15, 1.31] & 0.127 [0.089, 0.150] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 53.65 [51.89, 56.24] & 1.33 [1.30, 1.64] & 0.568 [0.512, 0.618] & 0.000 [0.000, 0.000] \\ 
Prollect & 96.7\% & 0.0\% & 52.75 [50.50, 56.95] & 1.24 [1.24, 1.26] & 0.020 [0.010, 0.030] & 0.039 [0.027, 0.049] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_cpp/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=0.99, lower quartile=0.99, median=0.99, upper quartile=0.99, upper whisker=0.99}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=55.10, median=55.50, upper quartile=56.35, upper whisker=56.55}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.41, median=1.42, upper quartile=1.43, upper whisker=1.47}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=57.10, lower quartile=57.55, median=58.95, upper quartile=60.20, upper whisker=60.40}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=0.92, lower quartile=1.04, median=1.06, upper quartile=1.10, upper whisker=1.41}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=54.20, median=54.90, upper quartile=55.10, upper whisker=55.15}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.23, median=1.24, upper quartile=1.24, upper whisker=1.24}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=48.35, lower quartile=49.85, median=51.35, upper quartile=51.35, upper whisker=53.15}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.42, lower quartile=1.42, median=1.43, upper quartile=1.43, upper whisker=1.45}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=49.45, lower quartile=50.55, median=51.70, upper quartile=53.10, upper whisker=53.25}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.26, lower quartile=1.26, median=1.63, upper quartile=1.64, upper whisker=1.69}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=47.70, lower quartile=48.15, median=51.35, upper quartile=51.45, upper whisker=52.75}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.23, lower quartile=1.24, median=1.24, upper quartile=1.24, upper whisker=1.28}}] coordinates {};


==> sim/results_cpp/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 100.0\% & -- & 0.99 [0.99, 0.99] & 0.555 [0.555, 0.555] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 55.50 [55.10, 56.35] & 1.42 [1.41, 1.43] & 0.031 [0.020, 0.040] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 20.0\% & 58.95 [57.55, 60.20] & 1.06 [1.04, 1.10] & 0.213 [0.181, 0.219] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.90 [54.20, 55.10] & 1.24 [1.23, 1.24] & 0.019 [0.018, 0.027] & 0.069 [0.036, 0.076] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 51.35 [49.85, 51.35] & 1.43 [1.42, 1.43] & 0.036 [0.029, 0.038] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 51.70 [50.55, 53.10] & 1.63 [1.26, 1.64] & 0.517 [0.500, 0.530] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 51.35 [48.15, 51.45] & 1.24 [1.24, 1.24] & 0.025 [0.019, 0.059] & 0.036 [0.026, 0.040] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_orca/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.26, lower quartile=1.26, median=1.26, upper quartile=1.26, upper whisker=1.26}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=54.02, median=54.70, upper quartile=55.41, upper whisker=56.55}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.41, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.24, lower quartile=1.27, median=1.28, upper quartile=1.29, upper whisker=1.31}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=57.10, lower quartile=58.35, median=58.85, upper quartile=59.95, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.29, upper quartile=1.29, upper whisker=1.41}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=54.20, median=54.42, upper quartile=54.81, upper whisker=55.15}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.23, median=1.24, upper quartile=1.24, upper whisker=1.25}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=50.11, median=51.35, upper quartile=52.90, upper whisker=59.10}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.42, lower quartile=1.43, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=55.10, lower quartile=62.15, median=69.20, upper quartile=76.25, upper whisker=83.30}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.28, upper quartile=1.29, upper whisker=1.36}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=49.45, lower quartile=50.67, median=52.42, upper quartile=54.41, upper whisker=59.25}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.29, lower quartile=1.30, median=1.36, upper quartile=1.57, upper whisker=1.69}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=47.70, lower quartile=48.84, median=51.40, upper quartile=52.55, upper whisker=56.95}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.23, lower quartile=1.24, median=1.24, upper quartile=1.25, upper whisker=1.28}}] coordinates {};


==> sim/results_orca/latex_scaling_table.tex <==
% Auto-generated scaling table (\input{sim/results/latex_scaling_table.tex})
\begin{table*}[t]
\caption{Scaling study (parallel C++ simulator): median runtime per control call (\,$\mu$s) and completion rate (\%); each cell aggregates 5 Monte Carlo seeds.}
\centering\scriptsize
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}\toprule
Scenario & $N$ & VO $\mu$s / Comp & ORCA $\mu$s / Comp & DMPC $\mu$s / Comp & Prollect $\mu$s / Comp \\ \midrule
intersection & 20 & 3.12 / 0.0 & 2.54 / 0.0 & 2.87 / 0.0 & 2.64 / 100.0 \\ 
intersection & 40 & 4.22 / 0.0 & 4.00 / 0.0 & 4.12 / 0.0 & 3.94 / 100.0 \\ 
intersection & 80 & 6.52 / 0.0 & 5.61 / 0.0 & 5.06 / 100.0 & 4.89 / 100.0 \\ 
\midrule
bottleneck & 16 & 2.60 / 100.0 & 2.59 / 0.0 & 2.20 / 100.0 & 2.42 / 100.0 \\ 
bottleneck & 32 & 4.20 / 100.0 & 4.31 / 0.0 & 3.84 / 20.0 & 4.68 / 100.0 \\ 
bottleneck & 64 & 7.21 / 60.0 & 7.97 / 0.0 & 6.60 / 0.0 & 7.20 / 100.0 \\ 
\midrule
random & 20 & 1.63 / 100.0 & 1.96 / 40.0 & 1.58 / 100.0 & 1.85 / 100.0 \\ 
random & 40 & 3.06 / 100.0 & 3.52 / 0.0 & 3.29 / 100.0 & 3.38 / 100.0 \\ 
random & 80 & 5.65 / 60.0 & 7.10 / 0.0 & 6.31 / 100.0 & 5.59 / 60.0 \\ 
\bottomrule\end{tabular}
\label{tab:scaling}
\end{table*}


==> sim/results_orca/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.26 [1.26, 1.26] & 0.487 [0.487, 0.487] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.70 [54.02, 55.41] & 1.43 [1.41, 1.44] & 0.025 [0.014, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.28 [1.27, 1.29] & 0.729 [0.713, 0.745] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.85 [58.35, 59.95] & 1.29 [1.28, 1.29] & 0.208 [0.186, 0.219] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.42 [54.20, 54.81] & 1.24 [1.23, 1.24] & 0.021 [0.014, 0.026] & 0.073 [0.067, 0.087] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 51.35 [50.11, 52.90] & 1.43 [1.43, 1.44] & 0.032 [0.015, 0.042] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 20.0\% & 0.0\% & 69.20 [62.15, 76.25] & 1.28 [1.27, 1.29] & 0.578 [0.520, 0.656] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 52.42 [50.67, 54.41] & 1.36 [1.30, 1.57] & 0.526 [0.504, 0.598] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 51.40 [48.84, 52.55] & 1.24 [1.24, 1.25] & 0.021 [0.010, 0.025] & 0.032 [0.026, 0.040] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_orca_safe/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - completion_time
\addplot[boxplot prepared={{lower whisker=81.90, lower quartile=81.90, median=81.90, upper quartile=81.90, upper whisker=81.90}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.15, lower quartile=1.15, median=1.15, upper quartile=1.15, upper whisker=1.15}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=54.02, median=54.70, upper quartile=55.41, upper whisker=56.55}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.41, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.13, lower quartile=1.14, median=1.15, upper quartile=1.18, upper whisker=1.32}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=57.10, lower quartile=58.35, median=58.85, upper quartile=59.95, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.29, upper quartile=1.29, upper whisker=1.41}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=54.20, median=54.42, upper quartile=54.81, upper whisker=55.15}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.23, median=1.24, upper quartile=1.24, upper whisker=1.25}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=50.11, median=51.35, upper quartile=52.90, upper whisker=59.10}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.42, lower quartile=1.43, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=50.50, median=51.40, upper quartile=54.70, upper whisker=62.15}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.13, lower quartile=1.15, median=1.15, upper quartile=1.27, upper whisker=1.41}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=49.45, lower quartile=50.67, median=52.42, upper quartile=54.41, upper whisker=59.25}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.29, lower quartile=1.30, median=1.36, upper quartile=1.57, upper whisker=1.69}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=47.70, lower quartile=48.84, median=51.40, upper quartile=52.55, upper whisker=56.95}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.23, lower quartile=1.24, median=1.24, upper quartile=1.25, upper whisker=1.28}}] coordinates {};


==> sim/results_orca_safe/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 100.0\% & 0.0\% & 81.90 [81.90, 81.90] & 1.15 [1.15, 1.15] & 0.134 [0.134, 0.134] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.70 [54.02, 55.41] & 1.43 [1.41, 1.44] & 0.025 [0.014, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.15 [1.14, 1.18] & 0.490 [0.469, 0.525] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.85 [58.35, 59.95] & 1.29 [1.28, 1.29] & 0.208 [0.186, 0.219] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.42 [54.20, 54.81] & 1.24 [1.23, 1.24] & 0.021 [0.014, 0.026] & 0.073 [0.067, 0.087] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 51.35 [50.11, 52.90] & 1.43 [1.43, 1.44] & 0.032 [0.015, 0.042] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 90.0\% & 0.0\% & 51.40 [50.50, 54.70] & 1.15 [1.15, 1.27] & 0.120 [0.091, 0.144] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 52.42 [50.67, 54.41] & 1.36 [1.30, 1.57] & 0.526 [0.504, 0.598] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 51.40 [48.84, 52.55] & 1.24 [1.24, 1.25] & 0.021 [0.010, 0.025] & 0.032 [0.026, 0.040] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_orca_smoke/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=0.99, lower quartile=0.99, median=0.99, upper quartile=0.99, upper whisker=0.99}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=0.99, lower quartile=0.99, median=0.99, upper quartile=0.99, upper whisker=0.99}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=55.10, median=55.50, upper quartile=56.35, upper whisker=56.55}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.41, median=1.42, upper quartile=1.43, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=0.92, lower quartile=0.92, median=0.94, upper quartile=0.96, upper whisker=1.02}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=57.10, lower quartile=57.55, median=58.95, upper quartile=60.20, upper whisker=60.40}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=0.92, lower quartile=1.04, median=1.06, upper quartile=1.10, upper whisker=1.41}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=54.20, median=54.90, upper quartile=55.10, upper whisker=55.15}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.23, median=1.24, upper quartile=1.24, upper whisker=1.24}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=48.35, lower quartile=49.85, median=51.35, upper quartile=51.35, upper whisker=53.15}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.42, lower quartile=1.42, median=1.43, upper quartile=1.43, upper whisker=1.45}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=61.20, lower quartile=65.92, median=70.65, upper quartile=74.30, upper whisker=77.95}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.04, lower quartile=1.06, median=1.25, upper quartile=1.25, upper whisker=1.30}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=49.45, lower quartile=50.55, median=51.70, upper quartile=53.10, upper whisker=53.25}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.26, lower quartile=1.26, median=1.63, upper quartile=1.64, upper whisker=1.69}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=47.70, lower quartile=48.15, median=51.35, upper quartile=51.45, upper whisker=52.75}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.23, lower quartile=1.24, median=1.24, upper quartile=1.24, upper whisker=1.28}}] coordinates {};


==> sim/results_orca_smoke/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 100.0\% & -- & 0.99 [0.99, 0.99] & 0.421 [0.421, 0.421] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 100.0\% & -- & 0.99 [0.99, 0.99] & 0.555 [0.555, 0.555] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 55.50 [55.10, 56.35] & 1.42 [1.41, 1.43] & 0.031 [0.020, 0.040] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 80.0\% & -- & 0.94 [0.92, 0.96] & 0.640 [0.620, 0.652] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 20.0\% & 58.95 [57.55, 60.20] & 1.06 [1.04, 1.10] & 0.213 [0.181, 0.219] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.90 [54.20, 55.10] & 1.24 [1.23, 1.24] & 0.019 [0.018, 0.027] & 0.069 [0.036, 0.076] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 51.35 [49.85, 51.35] & 1.43 [1.42, 1.43] & 0.036 [0.029, 0.038] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 60.0\% & 0.0\% & 70.65 [65.92, 74.30] & 1.25 [1.06, 1.25] & 0.419 [0.377, 0.630] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 51.70 [50.55, 53.10] & 1.63 [1.26, 1.64] & 0.517 [0.500, 0.530] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 51.35 [48.15, 51.45] & 1.24 [1.24, 1.24] & 0.025 [0.019, 0.059] & 0.036 [0.026, 0.040] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_orca_tuned/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.03, lower quartile=1.03, median=1.03, upper quartile=1.03, upper whisker=1.03}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=54.02, median=54.70, upper quartile=55.41, upper whisker=56.55}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.40, lower quartile=1.41, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% bottleneck / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.03, lower quartile=1.05, median=1.13, upper quartile=1.18, upper whisker=1.35}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=57.10, lower quartile=58.35, median=58.85, upper quartile=59.95, upper whisker=60.95}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.28, median=1.29, upper quartile=1.29, upper whisker=1.41}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=54.20, median=54.42, upper quartile=54.81, upper whisker=55.15}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.23, median=1.24, upper quartile=1.24, upper whisker=1.25}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=47.85, lower quartile=50.11, median=51.35, upper quartile=52.90, upper whisker=59.10}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.42, lower quartile=1.43, median=1.43, upper quartile=1.44, upper whisker=1.47}}] coordinates {};
% random / orca - completion_time
\addplot[boxplot prepared={{lower whisker=50.45, lower quartile=51.96, median=54.20, upper quartile=58.57, upper whisker=64.75}}] coordinates {};
% random / orca - min_distance
\addplot[boxplot prepared={{lower whisker=1.00, lower quartile=1.06, median=1.08, upper quartile=1.17, upper whisker=1.30}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=49.45, lower quartile=50.67, median=52.42, upper quartile=54.41, upper whisker=59.25}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.29, lower quartile=1.30, median=1.36, upper quartile=1.57, upper whisker=1.69}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=47.70, lower quartile=48.84, median=51.40, upper quartile=52.55, upper whisker=56.95}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.23, lower quartile=1.24, median=1.24, upper quartile=1.25, upper whisker=1.28}}] coordinates {};


==> sim/results_orca_tuned/latex_scaling_table.tex <==
% Auto-generated scaling table (\input{sim/results/latex_scaling_table.tex})
\begin{table*}[t]
\caption{Scaling study (parallel C++ simulator): median runtime per control call (\,$\mu$s) and completion rate (\%); each cell aggregates 5 Monte Carlo seeds.}
\centering\scriptsize
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}\toprule
Scenario & $N$ & VO $\mu$s / Comp & ORCA $\mu$s / Comp & DMPC $\mu$s / Comp & Prollect $\mu$s / Comp \\ \midrule
intersection & 20 & 3.75 / 0.0 & 1.76 / 0.0 & 3.52 / 0.0 & 3.01 / 100.0 \\ 
intersection & 40 & 4.67 / 0.0 & 2.50 / 0.0 & 4.62 / 0.0 & 4.30 / 100.0 \\ 
intersection & 80 & 6.35 / 0.0 & 3.27 / 0.0 & 5.09 / 100.0 & 5.43 / 100.0 \\ 
\midrule
bottleneck & 16 & 2.56 / 100.0 & 1.73 / 0.0 & 3.41 / 100.0 & 2.87 / 100.0 \\ 
bottleneck & 32 & 4.54 / 100.0 & 2.87 / 0.0 & 3.94 / 20.0 & 4.53 / 100.0 \\ 
bottleneck & 64 & 7.17 / 60.0 & 4.82 / 0.0 & 7.48 / 0.0 & 8.84 / 100.0 \\ 
\midrule
random & 20 & 1.89 / 100.0 & 1.33 / 100.0 & 1.72 / 100.0 & 2.21 / 100.0 \\ 
random & 40 & 3.06 / 100.0 & 2.18 / 60.0 & 3.08 / 100.0 & 3.50 / 100.0 \\ 
random & 80 & 6.13 / 60.0 & 4.48 / 20.0 & 6.19 / 100.0 & 5.89 / 60.0 \\ 
\bottomrule\end{tabular}
\label{tab:scaling}
\end{table*}


==> sim/results_orca_tuned/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.03 [1.03, 1.03] & 0.171 [0.171, 0.171] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.70 [54.02, 55.41] & 1.43 [1.41, 1.44] & 0.025 [0.014, 0.032] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 0.0\% & 0.0\% & -- & 1.13 [1.05, 1.18] & 0.487 [0.462, 0.503] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 58.85 [58.35, 59.95] & 1.29 [1.28, 1.29] & 0.208 [0.186, 0.219] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.42 [54.20, 54.81] & 1.24 [1.23, 1.24] & 0.021 [0.014, 0.026] & 0.073 [0.067, 0.087] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 51.35 [50.11, 52.90] & 1.43 [1.43, 1.44] & 0.032 [0.015, 0.042] & 0.000 [0.000, 0.000] \\ 
Reactive ORCA & 100.0\% & 0.0\% & 54.20 [51.96, 58.57] & 1.08 [1.06, 1.17] & 0.127 [0.098, 0.149] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 52.42 [50.67, 54.41] & 1.36 [1.30, 1.57] & 0.526 [0.504, 0.598] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 51.40 [48.84, 52.55] & 1.24 [1.24, 1.25] & 0.021 [0.010, 0.025] & 0.032 [0.026, 0.040] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}



==> sim/results_smoke/latex_boxplots.tex <==
% Auto-generated boxplot data for manuscript
% Usage: \\addplot[boxplot prepared={...}] coordinates {...};

% intersection / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.39, lower quartile=1.39, median=1.39, upper quartile=1.39, upper whisker=1.39}}] coordinates {};
% intersection / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.27, lower quartile=1.27, median=1.27, upper quartile=1.27, upper whisker=1.27}}] coordinates {};
% intersection / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=69.25, lower quartile=69.25, median=69.25, upper quartile=69.25, upper whisker=69.25}}] coordinates {};
% intersection / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.22, lower quartile=1.22, median=1.22, upper quartile=1.22, upper whisker=1.22}}] coordinates {};
% bottleneck / vo - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=53.67, median=54.15, upper quartile=54.62, upper whisker=55.10}}] coordinates {};
% bottleneck / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.42, lower quartile=1.43, median=1.45, upper quartile=1.46, upper whisker=1.47}}] coordinates {};
% bottleneck / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=57.10, lower quartile=57.22, median=57.35, upper quartile=57.47, upper whisker=57.60}}] coordinates {};
% bottleneck / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.29, lower quartile=1.32, median=1.35, upper quartile=1.38, upper whisker=1.41}}] coordinates {};
% bottleneck / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=53.20, lower quartile=53.62, median=54.05, upper quartile=54.47, upper whisker=54.90}}] coordinates {};
% bottleneck / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.23, lower quartile=1.24, median=1.24, upper quartile=1.24, upper whisker=1.24}}] coordinates {};
% random / vo - completion_time
\addplot[boxplot prepared={{lower whisker=51.35, lower quartile=51.80, median=52.25, upper quartile=52.70, upper whisker=53.15}}] coordinates {};
% random / vo - min_distance
\addplot[boxplot prepared={{lower whisker=1.43, lower quartile=1.44, median=1.44, upper quartile=1.44, upper whisker=1.45}}] coordinates {};
% random / dmpc - completion_time
\addplot[boxplot prepared={{lower whisker=53.15, lower quartile=53.17, median=53.20, upper quartile=53.22, upper whisker=53.25}}] coordinates {};
% random / dmpc - min_distance
\addplot[boxplot prepared={{lower whisker=1.29, lower quartile=1.30, median=1.30, upper quartile=1.30, upper whisker=1.30}}] coordinates {};
% random / prollect - completion_time
\addplot[boxplot prepared={{lower whisker=51.45, lower quartile=51.77, median=52.10, upper quartile=52.42, upper whisker=52.75}}] coordinates {};
% random / prollect - min_distance
\addplot[boxplot prepared={{lower whisker=1.23, lower quartile=1.23, median=1.24, upper quartile=1.24, upper whisker=1.24}}] coordinates {};


==> sim/results_smoke/latex_scaling_table.tex <==
% Auto-generated scaling table (\input{sim/results/latex_scaling_table.tex})
\begin{table*}[t]
\caption{Scaling study (parallel C++ simulator): median runtime per control call (\,$\mu$s) and completion rate (\%); each cell aggregates 2 Monte Carlo seeds.}
\centering\scriptsize
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}\toprule
Scenario & $N$ & VO $\mu$s / Comp & DMPC $\mu$s / Comp & Prollect $\mu$s / Comp \\ \midrule
intersection & 20 & 2.56 / 0.0 & 2.08 / 0.0 & 1.94 / 100.0 \\ 
intersection & 40 & 4.58 / 0.0 & 4.71 / 0.0 & 4.48 / 100.0 \\ 
intersection & 80 & 6.74 / 0.0 & 4.91 / 100.0 & 5.06 / 100.0 \\ 
\midrule
bottleneck & 16 & 2.60 / 100.0 & 2.52 / 100.0 & 2.49 / 100.0 \\ 
bottleneck & 32 & 4.10 / 100.0 & 3.90 / 50.0 & 4.30 / 100.0 \\ 
bottleneck & 64 & 7.04 / 50.0 & 6.71 / 0.0 & 7.51 / 100.0 \\ 
\midrule
random & 20 & 1.88 / 100.0 & 1.63 / 100.0 & 2.05 / 100.0 \\ 
random & 40 & 2.96 / 100.0 & 3.21 / 100.0 & 3.45 / 100.0 \\ 
random & 80 & 5.54 / 50.0 & 5.76 / 100.0 & 5.50 / 50.0 \\ 
\bottomrule\end{tabular}
\label{tab:scaling}
\end{table*}


==> sim/results_smoke/latex_tables.tex <==
% Auto-generated LaTeX tables (\input{sim/results/latex_tables.tex})

\begin{table*}[t]
\caption{Intersection results (30 runs): median [IQR] where applicable}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 0.0\% & 0.0\% & -- & 1.39 [1.39, 1.39] & 0.978 [0.978, 0.978] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 0.0\% & 0.0\% & -- & 1.27 [1.27, 1.27] & 0.578 [0.578, 0.578] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 69.25 [69.25, 69.25] & 1.22 [1.22, 1.22] & 0.066 [0.066, 0.066] & 0.063 [0.063, 0.063] \\ 
\bottomrule
\end{tabular}
\label{tab:intersection_eff}
\end{table*}

\begin{table*}[t]
\caption{Bottleneck results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 54.15 [53.67, 54.62] & 1.45 [1.43, 1.46] & 0.019 [0.014, 0.025] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 57.35 [57.22, 57.47] & 1.35 [1.32, 1.38] & 0.176 [0.173, 0.179] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 54.05 [53.62, 54.47] & 1.24 [1.24, 1.24] & 0.018 [0.013, 0.022] & 0.029 [0.026, 0.032] \\ 
\bottomrule
\end{tabular}
\label{tab:bottleneck_eff}
\end{table*}

\begin{table*}[t]
\caption{Random waypoint results (30 runs): median [IQR]}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Method & Comp. & Coll. & Time (s) & Min Dist. (m) & $\overline{\Delta v}$ & Preempt \\ \midrule
Reactive VO & 100.0\% & 0.0\% & 52.25 [51.80, 52.70] & 1.44 [1.44, 1.44] & 0.056 [0.046, 0.066] & 0.000 [0.000, 0.000] \\ 
DMPC-like & 100.0\% & 0.0\% & 53.20 [53.17, 53.22] & 1.30 [1.30, 1.30] & 0.537 [0.499, 0.576] & 0.000 [0.000, 0.000] \\ 
Prollect & 100.0\% & 0.0\% & 52.10 [51.77, 52.42] & 1.24 [1.23, 1.24] & 0.076 [0.067, 0.084] & 0.053 [0.047, 0.060] \\ 
\bottomrule
\end{tabular}
\label{tab:random_eff}
\end{table*}


